Allocating Variance to Maximize Expectation

We design efficient approximation algorithms for maximizing the expectation of the supremum of families of Gaussian random variables. In particular, let $\mathrm{OPT}:=\max_{\sigma_1,\cdots,\sigma_n}\mathbb{E}\left[\sum_{j=1}^{m}\max_{i\in S_j} X_i\right]$, where $X_i$ are Gaussian, $S_j\subset[n]$ and $\sum_i\sigma_i^2=1$, then our theoretical results include: - We characterize the optimal variance allocation -- it concentrates on a small subset of variables as $|S_j|$ increases, - A polynomial time approximation scheme (PTAS) for computing $\mathrm{OPT}$ when $m=1$, and - An $O(\log n)$ approximation algorithm for computing $\mathrm{OPT}$ for general $m>1$. Such expectation maximization problems occur in diverse applications, ranging from utility maximization in auctions markets to learning mixture models in quantitative genetics.

==> macros.tex <==
\newcommand\now{\mathsf{now}}
\newcommand\pre{\mathsf{pre}}
\newcommand\maxSum{\mathsf{maxSum}}
\newcommand\minSum{\mathsf{minSum}}
\newcommand\totalSum{\mathsf{totalSum}}

\renewcommand\v{\vec v}
\renewcommand\u{\vec u}
\renewcommand\b{\vec b}
\newcommand\bmb[2]{\vec b^{(#1, #2)}}
\newcommand\bmv[2]{\vec v^{(#1, #2)}}
\newcommand\p{\vec p}
\newcommand\vp{v^{\mathsf{pre}}}
\newcommand\hvp{\hat{v}^{\mathsf{pre}}}
\newcommand\vvp{\vec v^{\mathsf{pre}}}
\newcommand\vn{v^{\mathsf{now}}}
\newcommand\vnmax{v^{\mathsf{now}}_{\mathsf{max}}}
\newcommand\vvn{\vec v^{\mathsf{now}}}
\newcommand\x{\vec x}
\newcommand\y{\vec y}
\newcommand\R{\mathbb R}
\newcommand\X{\mathcal X}
\newcommand\cu{\overline U}
\newcommand\I{\mathcal I}
\renewcommand\P{\mathcal P}
\newcommand{\f}{f}
\newcommand\V{\mathcal V}
\newcommand\K{\mathcal K}
\newcommand\A{\mathcal A}
\renewcommand\S{\mathcal S}
\renewcommand\H{\mathcal H}
\newcommand\barS{\overline{S}}
\newcommand{\sat}{s}

\newcommand\Rev{\mathsf{Rev}}
\newcommand\Loss{\mathsf{Loss}}
\newcommand\OPT{\mathsf{OPT}}
\newcommand\opt{\mathsf{opt}}
\newcommand\sub{\mathsf{sub}}
\newcommand\other{\mathsf{other}}
\newcommand\same{\mathsf{same}}
\newcommand\change{\mathsf{change}}
\newcommand\base{\mathsf{base}}
\newcommand\summax{\mathsf{sum\mbox{-}max}}
\newcommand\subC{\mathsf{sub\mbox{-}L_0}}
\newcommand\rank{\mathsf{rank}}
\newcommand\crank{\mathsf{circuit\mbox{-}rank}}
\newcommand\circuit{\mathsf{circuit}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{lemma*}{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{mechanism}[theorem]{Mechanism}
\newtheorem{optimization}[theorem]{Optimization Problem}
\newtheorem{conjecture}[theorem]{Conjecture}

\newcommand{\N}{\mathcal{N}}

\newcommand{\e}{\epsilon}
\newcommand{\eps}{\epsilon}

\newcommand{\ret}{\mathcal{R}}
\newcommand{\alg}{\textsc{ALG}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\opt}{\textsc{OPT}}
\newcommand{\ub}{\textsc{UB}}
\newcommand{\lb}{\textsc{LB}}
\newcommand{\ratio}{\textsc{R}}
\newcommand{\si}{SR }

\newcommand{\dist}{D}
\newcommand{\adx}{AdEx\xspace}
\newcommand{\gam}{\gamma}


\usepackage{color}
\newcounter{note}[section]
\newcommand{\ynote}[1]{\refstepcounter{note}$\ll${\bf Yifeng~\thenote:}
  {\sf \color{blue}  #1}$\gg$\marginpar{\tiny\bf YT~\thenote}}

\SetKwComment{Comment}{/* }{ */}
